Model2Scene: Learning 3D Scene Representation via Contrastive Language-CAD Models Pre-training

Current successful methods of 3D scene perception rely on the large-scale annotated point cloud, which is tedious and expensive to acquire. In this paper, we propose Model2Scene, a novel paradigm that learns free 3D scene representation from Computer-Aided Design (CAD) models and languages. The main challenges are the domain gaps between the CAD models and the real scene's objects, including model-to-scene (from a single model to the scene) and synthetic-to-real (from synthetic model to real scene's object). To handle the above challenges, Model2Scene first simulates a crowded scene by mixing data-augmented CAD models. Next, we propose a novel feature regularization operation, termed Deep Convex-hull Regularization (DCR), to project point features into a unified convex hull space, reducing the domain gap. Ultimately, we impose contrastive loss on language embedding and the point features of CAD models to pre-train the 3D network. Extensive experiments verify the learned 3D scene representation is beneficial for various downstream tasks, including label-free 3D object salient detection, label-efficient 3D scene perception and zero-shot 3D semantic segmentation. Notably, Model2Scene yields impressive label-free 3D object salient detection with an average mAP of 46.08\% and 55.49\% on the ScanNet and S3DIS datasets, respectively. The code will be publicly available.

==> future.tex <==
\section{Future Work}


\begin{itemize}
\item {\textbf{training with multiple GPUs}}
\item {\textbf{add full classes.}}
\item {\textbf{add more datasets.}}
\item {add virtual scanning}
\item {\textbf{zero-shot setting. During infering time. given unseen referring models, localize the same semantic objects in an unseen scene}}
\item {visualization of prototypes}
\item {more downstream tasks}
\item {visualization of data processing}
\item {T-SNE visualization}
\item {Teacher student network, teacher for virtual data, student for real data}
\item {herchial memory for inner class and inter class}
\item {adjust temperature to synthe new features}
\item {reuse the classifier to fine-tune}
\item {voxel transformer}
\item {contrastive learning between models}

\end{itemize}
